A software toolkit and hardware platform for investigating and comparing robot autonomy algorithms in simulation and reality

We describe a software framework and a hardware platform used in tandem for the design and analysis of robot autonomy algorithms in simulation and reality. The software, which is open source, containerized, and operating system (OS) independent, has three main components: a ROS 2 interface to a C++ vehicle simulation framework (Chrono), which provides high-fidelity wheeled/tracked vehicle and sensor simulation; a basic ROS 2-based autonomy stack for algorithm design and testing; and, a development ecosystem which enables visualization, and hardware-in-the-loop experimentation in perception, state estimation, path planning, and controls. The accompanying hardware platform is a 1/6th scale vehicle augmented with reconfigurable mountings for computing, sensing, and tracking. Its purpose is to allow algorithms and sensor configurations to be physically tested and improved. Since this vehicle platform has a digital twin within the simulation environment, one can test and compare the same algorithms and autonomy stack in simulation and reality. This platform has been built with an eye towards characterizing and managing the simulation-to-reality gap. Herein, we describe how this platform is set up, deployed, and used to improve autonomy for mobility applications.

==> sections/usage.tex <==
%!TEX root = ../root.tex

As this contribution highlights a research platform, we foresee a multitude of opportunities for the community to leverage this platform. First, we have developed this platform such that we can leverage this environment and platform to conduct research into the difference between simulation and reality. With that in mind, both ART and the digital twin will be equipped with additional sensors (e.g. GPS, IMU, and extra cameras including a stereo camera). With this platform, one can track the position of the vehicle in reality via a motion capture system. Similarly the position of the vehicle can be monitored in simulation. With this information, the behavior, paths, and reactions of the vehicle when run in simulation can be compared with those in reality. Second, ATK can be used by researchers and other organizations to facilitate autonomy algorithm development by allowing them to configure a custom set of containers to host their development, deployment, simulation, and visualization. We anticipate UW Madison's Wisconsin Autonomous will use this platform to assist in their Autodrive Competition. In addition, we foresee an opportunity for researchers looking into specific components of the autonomy stack to leverage this platform to consider multiple algorithms and replace just those components within the autonomy stack. For example, a planning researcher can leverage the perception components of the current and future ART developments to build planning without needing to dedicate time and resources toward configuring the sensors, the perception algorithms, and the development/deployment environment. Another foreseen use of the environment is to conduct hardware in the loop testing. By allowing the container to be deployed on multiple systems (e.g. the simulation on a remote server and the development environment on the ART vehicle), hardware in the loop can be evaluated. While the simulation cannot guarantee hard real time performance, it can be setup in a way where soft real time simulation is enabled. Various hardware architectures and configurations can then be compared within ART. 


